Backwards Reachability for Probabilistic Timed Automata: A Replication Report

Backwards reachability is an efficient zone-based approach for model checking probabilistic timed automata w.r.t. PTCTL properties. Current implementations, however, are restricted to maximum probabilities of reachability properties. In this paper, we report on our new implementation of backwards reachability as part of the Modest Toolset. Its support for minimum and maximum probabilities of until formulas makes it the most general implementation available today. We compare its behaviour to the experimental results reported in the original papers presenting the backwards reachability technique.

==> data.runtime.tex <==
\pgfplotstableread[col sep=semicolon]{
%
modeltype;setupbr;setupdc;
aodvRERR;12.891;9.8;
brp-pta-max;0.365;0.1;
brp-pta-min;1000;0.1;
firewire-pta;0.241;1000;
firewire-pta;0.245;1000;
firewire-pta;1000;1000;
firewire-pta;0.237;1000;
firewire-pta;0.237;1000;
firewire-pta;1000;1000;
firewire-pta;1000;1000;
firewire-pta;0.245;1000;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
firewire_abst-pta;0.1;0.1;
zeroconf-pta;0.1;0.1;
zeroconf-pta;0.1;0.1;
zeroconf-pta;0.1;0.1;
zeroconf-pta;0.1;0.1;


}\pspdatasetup%


\pgfplotstableread[col sep=semicolon]{
%
modeltype;property;goal;checkbr;checkdc;
aodvRERR;RrtNextHop_1_4_short;Maximum;0.1;9.8;
aodvRERR;RrtNextHop_1_4_long;Maximum;0.1;9.8;
aodvRERR;sanity_check;Maximum;0.1;9.8;
aodvRERR;delivery;Maximum;0.1;9.8;
brp-pta-max;T_1;Maximum;0.587;0.1;
brp-pta-max;T_2;Maximum;0.406;0.1;
brp-pta-max;T_A1;Maximum;0.372;0.1;
brp-pta-max;T_A2;Maximum;0.1;0.1;
brp-pta-max;P_A;Maximum;0.1;0.1;
brp-pta-max;P_B;Maximum;0.1;0.1;
brp-pta-max;P_1;Maximum;1.017;0.1;
brp-pta-max;P_2;Maximum;0.145;0.1;
brp-pta-max;P_3;Maximum;0.264;0.1;
brp-pta-max;P_4;Maximum;0.1;0.1;
brp-pta-max;Dmax;Maximum;33.988;0.1;
brp-pta-min;Dmin;Minimum;1000;0.1;
firewire_abst-pta;deadline_max;Maximum;0.1;0.1;
firewire_abst-pta;deadline_min;Minimum;0.1;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;0.358;0.1;
firewire_abst-pta;deadline_min;Minimum;0.373;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;1.858;0.1;
firewire_abst-pta;deadline_min;Minimum;1.51;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;0.1;0.1;
firewire_abst-pta;deadline_min;Minimum;0.1;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;0.1;0.1;
firewire_abst-pta;deadline_min;Minimum;0.1;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;0.394;0.1;
firewire_abst-pta;deadline_min;Minimum;0.151;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;2.046;0.1;
firewire_abst-pta;deadline_min;Minimum;0.446;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
firewire_abst-pta;deadline_max;Maximum;0.1;0.1;
firewire_abst-pta;deadline_min;Minimum;0.1;0.1;
firewire_abst-pta;eventually;Minimum;0.1;0.1;
zeroconf-pta;deadline;Maximum;0.1;0.1;
zeroconf-pta;incorrect;Maximum;0.1;0.1;
zeroconf-pta;deadline;Maximum;0.1;0.1;
zeroconf-pta;incorrect;Maximum;0.1;0.1;
zeroconf-pta;deadline;Maximum;0.367;0.1;
zeroconf-pta;incorrect;Maximum;0.1;0.1;
zeroconf-pta;deadline;Maximum;6.771;0.1;
zeroconf-pta;incorrect;Maximum;0.1;0.1;


}\pspdatacheck%


\pgfplotstableread[col sep=semicolon]{
%
modeltype;timebr;timedc;
aodvRERR;13.075;49.0;
brp-pta-max;37.268;1.2;
brp-pta-min;1000;0.1;
firewire-pta;0.241;1000;
firewire-pta;0.245;1000;
firewire-pta;1000;1000;
firewire-pta;0.237;1000;
firewire-pta;0.237;1000;
firewire-pta;1000;1000;
firewire-pta;1000;1000;
firewire-pta;0.245;1000;
firewire_abst-pta;0.229;0.1;
firewire_abst-pta;0.82;0.1;
firewire_abst-pta;3.462;0.1;
firewire_abst-pta;0.154;0.1;
firewire_abst-pta;0.19899999999999998;0.4;
firewire_abst-pta;0.639;0.4;
firewire_abst-pta;2.584;0.4;
firewire_abst-pta;0.14100000000000001;0.4;
zeroconf-pta;0.1;0.1;
zeroconf-pta;0.1;0.1;
zeroconf-pta;0.435;0.1;
zeroconf-pta;6.841;0.1;


}\pspdatatotal%
